Cosmology with Very-High-Energy Gamma Rays

In this chapter, we discuss the contributions of gamma-ray astronomy at TeV energies to our understanding of the visible content and structure of the universe. We start from the present epoch with the second most intense electromagnetic background field after the CMB: the extragalactic background light (EBL). The EBL is composed of all the light emitted by stars and galaxies since the beginning of reionization, including light absorbed and re-emitted by dust. As such, the EBL traces the history of radiating matter in the universe. We then further dive into the large voids of the universe to study the large-scale magnetic fields that should permeate them. These fields could originate from the onset of structure formation or early phase transitions, bringing us back to the infancy of the universe. We conclude by looking back to the elusive Planck time scale, where the standard models of cosmology and particle physics are no longer applicable. Observations with current-generation gamma-ray astronomy experiments have now started to scratch the surface of cosmology, as we will show in this chapter.

==> add/acro.tex <==
\newacronym{4fgl}{4FGL}{fourth Fermi Large Area Telescope catalog}
\newacronym{adc}{ADC}{Anaologue to Digital Converter}
\newacronym{agile}{AGILE}{{\sl Astro-rivelatore Gamma a
Immagini LEggero}}
\newacronym{agn}{AGN}{Active Galactic Nucleus}
\newacronym{alp}{ALP}{Axion-like Particle}
\newacronym{ann}{ANN}{Artificial Neural Network}
\newacronym{au}{AU}{Astronomical Unit}
\newacronym{bh}{BH}{Black Hole}
\newacronym{bdt}{BDT}{Boosted Decision Trees}
\newacronym{cangaroo}{CANGAROO}{Collaboration of Australia and Nippon (Japan) for a Gamma-Ray Observatory in the Outback}
\newacronym{ccd}{CCD}{Charged-Coupled Device}
\newacronym{cdm}{CDM}{Cold Dark Matter}
\newacronym{cgro}{CGRO}{Compton Gamma-Ray Observatory}
\newacronym{cmb}{CMB}{Cosmic Microwave Background}
\newacronym{cmz}{CMZ}{Central Molecular Zone}
\newacronym{cnn}{CNN}{Convolutional Neural Networks}
\newacronym{cp}{CP}{Charge-Parity}
\newacronym{cr}{CR}{Cosmic Rays}
\newacronym{cta}{CTA}{Cherenkov Telescope Array}
\newacronym{ctao}{CTAO}{Cherenkov Telescope Array Observatory}
\newacronym{dm}{DM}{Dark Matter}
\newacronym{drs}{DRS}{Domino Ring Sampler}
\newacronym{dsa}{DSA}{Diffuse Shock Acceleration}
\newacronym{eas}{EAS}{Extensive Air Shower}
\newacronym{ebl}{EBL}{Extragalactic Background Light}
\newacronym{egret}{EGRET}{Energetic Gamma-Ray Experiment Telescope}
\newacronym{fact}{FACT}{First G-APD Cherenkov Telescope}
\newacronym{fadc}{FADC}{Flash \acrshort{adc}}
\newacronym{fermilat}{Fermi-LAT}{Fermi-Large Area Telescope}
\newacronym{fermi}{Fermi}{Fermi Gamma-Ray Space Telescope}
\newacronym{fsrq}{FSRQ}{Flat Spectrum Radio Quasar}
\newacronym{fpga}{FPGA}{Field Programmable Gate Array}
\newacronym{liv}{LIV}{Lorentz Invariance Violation}
\newacronym{lmc}{LMC}{Large Magellanic Cloud}
\newacronym{g-apd}{G-APD}{Geiger-mode avalanche photodiode}
\newacronym{gbm}{GBM}{Gamma-ray Burst Monitor}
\newacronym{gc}{GC}{Galactic }
\newacronym{grb}{GRB}{Gamma-ray Burst}
\newacronym{hawc}{HAWC}{High Altitude Water Cherenkov}
\newacronym{he}{HE}{High Energy}
\newacronym{hegra}{HEGRA}{High Energy Gamma-Ray}
\newacronym{hess}{H.E.S.S.}{High Energy Stereoscopic System}
\newacronym{iact}{IACT}{Imaging Atmospheric Cherenkov Telescope}
\newacronym{imbh}{IMBH}{Intermediate Mass Black Holes}
\newacronym{ism}{ISM}{InterStellar Medium}
\newacronym{lhaaso}{LHAASO}{The Large High Altitude Air Shower Observatory}
\newacronym{lidar}{LIDAR}{LIght Detection And Ranging}
\newacronym{lsp}{LSP}{Light SUSY Particle}
\newacronym{lst}{LST}{Large Size Telescope}
\newacronym{mace}{MACE}{Major Atmospheric Cherenkov Experiment Telescope}
\newacronym{MACHOs}{MACHOs}{Massive Astrophysical Compact Halo Objects}
\newacronym{magic}{MAGIC}{Major Atmospheric Gamma-ray Imaging Cherenkov}
\newacronym{mc}{MC}{Monte Carlo}
\newacronym{mm}{MM}{Magnetic Monopole}
\newacronym{MoG}{MoG}{Modified Gravity}
\newacronym{MoND}{MoND}{Modified Newtonian Dynamics}
\newacronym{mw}{MW}{Milky Way}
\newacronym{ns}{NS}{Neutron Star}
\newacronym{nsb}{NSB}{Night Sky Background}
\newacronym{oss}{OSS}{Optical Support System}
\newacronym{qcd}{QCD}{Quantum Chromodynamics}
\newacronym{qlt}{QLT}{Quasi-Linear Theory}
\newacronym{pao}{PBH}{Pierre Auger Observatory}
\newacronym{pbh}{PBH}{Primordial Black Hole}
\newacronym{phe}{ph.e.}{photo-electron}
\newacronym{pmt}{PMT}{Photo-Multiplier Tubes}
\newacronym{psf}{PSF}{Point Spread Function}
\newacronym{pwn}{PWNe}{Pulsar Wind Nebulae}
\newacronym{rf}{RF}{Random Forest}
\newacronym{rms}{RMS}{Root Mean Square}
\newacronym{sca}{SCA}{Switched Capacitor Array}
\newacronym{sm}{SM}{Stanard Model}
\newacronym{sn}{SN}{SuperNova}
\newacronym{snr}{SNR}{SuperNova Remnant}
\newacronym{tactic}{TACTIC}{TeV Atmospheric Cherenkov Telescope with Imaging Camera}
\newacronym{swgo}{SWGO}{Southern Wide-field Gamma-ray Observatory}
\newacronym{uhecr}{UHECR}{Ultra High Energy Cosmic Ray}
\newacronym{veritas}{VERITAS}{Very Energetic Radiation Imaging Telescope Array System}
\newacronym{vhe}{VHE}{Very High Energy}
\newacronym{wimp}{WIMPs}{Weakly Interacting Slim Particles}


\usepackage{amsthm}

%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{exercise}[theorem]{Exercise}

\newenvironment{myboxedtext}[1]
  {\begin{eBox}\textcolor{ocre}{{\bfseries\small\sffamily#1~}}}
  {\hfill{\color{ocre}\tiny\ensuremath{\blacksquare}}\end{eBox}}        








==> add/settings.tex <==
\usepackage{comment}% added by M. Doro
\usepackage{longtable,caption}
\usepackage{enumitem} % Michele 

%DIF PREAMBLE EXTENSION ADDED BY LATEXDIFF
%DIF UNDERLINE PREAMBLE %DIF PREAMBLE
\RequirePackage[normalem]{ulem} %DIF PREAMBLE
\RequirePackage{color}\definecolor{RED}{rgb}{1,0,0}\definecolor{BLUE}{rgb}{0,0,1} %DIF PREAMBLE
\providecommand{\DIFadd}[1]{{\protect\color{blue}\uwave{#1}}} %DIF PREAMBLE
\providecommand{\DIFdel}[1]{{\protect\color{red}\sout{#1}}}                      %DIF PREAMBLE
%DIF SAFE PREAMBLE %DIF PREAMBLE
\providecommand{\DIFaddbegin}{} %DIF PREAMBLE
\providecommand{\DIFaddend}{} %DIF PREAMBLE
\providecommand{\DIFdelbegin}{} %DIF PREAMBLE
\providecommand{\DIFdelend}{} %DIF PREAMBLE
%DIF FLOATSAFE PREAMBLE %DIF PREAMBLE
\providecommand{\DIFaddFL}[1]{\DIFadd{#1}} %DIF PREAMBLE
\providecommand{\DIFdelFL}[1]{\DIFdel{#1}} %DIF PREAMBLE
\providecommand{\DIFaddbeginFL}{} %DIF PREAMBLE
\providecommand{\DIFaddendFL}{} %DIF PREAMBLE
\providecommand{\DIFdelbeginFL}{} %DIF PREAMBLE
\providecommand{\DIFdelendFL}{} %DIF PREAMBLE
%DIF END PREAMBLE EXTENSION ADDED BY LATEXDIFF


\usepackage{verbatim} % added by M. Doro
\usepackage[acronym]{glossaries}
\usepackage{graphicx}
%\usepackage{natbib}
\usepackage{mathtools, cuted}
\usepackage{amsmath,amssymb,esint}
\usepackage[sort&compress,comma,authoryear]{natbib}
\usepackage[colorlinks=true,allcolors=blue,bookmarks=true]{hyperref}

% ADDED BY MICHELE, MIGUEL


\newcommand{\gammaray}{gamma-ray}
\newcommand{\hess}{H.E.S.S.}
\newcommand{\hegra}{HEGRA}
\newcommand{\cta}{CTA}
\newcommand{\LAT}{\emph{Fermi}-LAT}
\newcommand{\xmm}{\emph{XMM}-Newton}
\newcommand{\chandra}{\emph{Chandra}}
\newcommand{\nustar}{\emph{NuStar}}
\newcommand{\apj}{ApJ}
\newcommand{\apjs}{ApJS}
\newcommand{\apjf}{The Astrophysical Journal}
\newcommand{\apjl}{ApJL}
\newcommand{\apjlf}{The Astrophysical Journal Letters}
\newcommand{\aap}{A\&A}
\newcommand{\aapf}{Astronomy \& Astrophysics}
\newcommand{\aapr}{A\&A~Rev.}
\newcommand{\apss}{Ap\&SS}
\newcommand{\aaprf}{Astronomy \& Astrophysics Reviews}
\newcommand{\araa}{Annual Rev. of Astron. and Astrophys.}
\newcommand{\araaf}{Annual Review of Astronomy and Astrophysics}
\newcommand{\nat}{Nature}
\newcommand{\science}{Science}
\newcommand{\ap}{Astrop. Phys. }
\newcommand{\apf}{Astroparticle Physics Journal }
%\newcommand{\ajf}{Astroparticle Journal}
\newcommand{\ijmpd}{Int. J. of Mod. Phys. D}
\newcommand{\ijmpdf}{International Journal of Modern Physics D}
\newcommand{\jcap}{J. Cosmology Astropart. Phys.}
\newcommand{\jcapf}{Journal of Cosmology and Astroparticle Physics}
\newcommand{\jhea}{J. High-Energy Astroph.}
\newcommand{\jheaf}{Journal of High Energy Astrophysics}
\newcommand{\mnras}{MNRAS}
\newcommand{\mnrasf}{Monthly Notices of the Royal Astronomical Society}
\newcommand{\nima}{Nucl. Instrum. and Meth. in Phys. Research A}
\newcommand{\nimaf}{Nuclear Instruments and Methods in Physics Research A}
\newcommand{\plb}{Phys. Let. B}
\newcommand{\plbf}{Physics Letter B}
\newcommand{\prd}{Phys.~Rev.~D}
\newcommand{\prdf}{Physical Review D}
\newcommand{\prl}{Phys.~Rev.~Letter}
\newcommand{\prlf}{Physical Review Letter}
\newcommand{\physrep}{Physics Reports}
\newcommand{\pasj}{Pub. of the ASJ}
\newcommand{\pasjf}{Publications of the Astronomical Society of Japan}
\newcommand{\pos}{PoS}
\newcommand{\posf}{Proc. of Science}
\newcommand{\ssr}{S Review}
\newcommand{\etal}{\emph{et al.}}
\newcommand{\coll}{Collaboration}
%% RM's definitions (to be removed later)
\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\bea{\begin{eqnarray}}
\def\eea{\end{eqnarray}}
\def\beas{\begin{eqnarray*}}
\def\eeas{\end{eqnarray*}}
\def\lb{\label}
\def\bom{\mbox{\boldmath $\omega$}}
\def\bphi{\mbox{\boldmath $\phi$}}
\def\bna{\mbox{\boldmath $\nabla$}}
\def\brho{\mbox{\boldmath $\rho$}}
\def\lie{\mbox{\pounds}}
\def\la{\langle}
\def\ra{\rangle}
\def\pa{\partial}
\def\sq{\sqrt }
\def\l{\lambda }
\def\ph{\phi }
\def\o{\omega}
\def\t{\tau }
\def\th{\theta }
\def\k{\kappa }
\def\p{\pi }
\def\Ph{\Phi }
\def\ps{\psi }
\def\Ps{\Psi }
\def\ch{\chi }
\def\d{\delta }
\def\a{\alpha}
\def\e{\epsilon }
\def\b{\beta}
\def\do{\dot }
\def\dag{\dagger }
\def\pr{\prime }
\def\ve{\vert }
\def\hsp5{\hspace{5mm}}
\def\h{\hat }
\def\dag{\dagger }
\def\bp{\begin{pmatrix}}
\def\ep{\end{pmatrix}}
\def\bv{\begin{vmatrix}}
\def\ev{\end{vmatrix}}
\def\ran{\rangle }
\def\lan{\langle }
\def\half{\frac {1}{2}}
\def\kno{\vert n^{(0)}\ran }
\def\bno{\lan n^{(0)} \vert }


\usepackage{colortbl}
\usepackage{esvect}
\newcommand{\aaa}{alpha}
\newcommand{\svUL}{\langle \sigma \mathit{v} \rangle^\mathrm{UL}}
\newcommand{\sv}{\langle \sigma \mathit{v} \rangle}
\newcommand{\svsvt}{\sv_\mathrm{svt}}
\newcommand{\svdsu}{\sv_{2.71}}
\newcommand{\aaasvt}{\aaa_\mathrm{svt}}
\newcommand{\aaadsu}{\aaa_{2.71}}
\newcommand{\hataaa}{\hat{\aaa}}
\newcommand{\hatsv}{\widehat{\langle \sigma \mathit{v} \rangle}}
\newcommand{\doublehatnu}{\doublehat{\bm{\nu}}}
\newcommand{\hatnu}{\hat{\bm{\nu}}}
\newcommand{\hatmu}{\hat{\bm{\mu}}}
\newcommand{\hattheta}{\hat{\bm{\theta}}}
\newcommand{\thetaann}{\theta_\mathrm{ann}}
\newcommand{\thetadec}{\theta_\mathrm{dec}}
\newcommand{\data}{\bm{\mathcal{D}}}
\newcommand{\lkl}{\mathcal{L}}
%\newcommand{\loglkl}{\mathcal{l}}
\newcommand{\loglkl}{\log\mathcal{L}}
\newcommand{\overbar}[1]{\mkern 3.5mu\overline{\mkern-3.5mu#1\mkern-3.5mu}\mkern 3.5mu}
\newcommand{\non}{{N_\mathrm{ON}}}
\newcommand{\noff}{{N_\mathrm{OFF}}}
\newcommand{\emin}{{E'_\mathrm{min}}}
\newcommand{\emax}{{E'_\mathrm{max}}}
\newcommand{\mdm}{m_\mathrm{DM}}
\newcommand{\tdm}{\tau_\mathrm{DM}}
\newcommand{\taudm}{\tau_\mathrm{DM}}
\newcommand{\tdmLL}{\tau_\mathrm{DM}^\mathrm{UL}}
\newcommand{\dom}{{\Delta\Omega}}
\newcommand{\aeff}{ A_\mathrm{eff}}
\newcommand{\barJ}{\bar{J}}
\newcommand{\bb}{b\bar{b}}
\newcommand{\WW}{W^+W^-}
\newcommand{\tautau}{\tau^+\tau^-}
\newcommand{\mumu}{\mu^+\mu^-}
\newcommand{\gammagamma}{\gamma\gamma}
\newcommand{\Jobs}{J_\mathrm{obs}}
\newcommand{\Jobsi}{J_\mathrm{obs,i}}
\newcommand{\Dobs}{D_\mathrm{obs}}
\newcommand{\Dobsi}{D_\mathrm{obs,i}}
\newcommand{\lp}{\lambda_P}
\newcommand{\Junits}{GeV$^2$ cm$^{-5}$}
\newcommand{\Jdecunits}{GeV cm$^{-2}$}
\newcommand{\svunits}{cm$^3$ s$^{-1}$}
\newcommand{\Fermi}{\textit{Fermi}\xspace}
\newcommand{\Tobsi}{T_{\mathrm{obs},i}}
\newcommand{\triangulum}{Tri~II\xspace}
\newcommand{\ppterm}{\frac{d\overline{\Phi}_\textrm{PP}}{dE}}
\newcommand{\ppdecterm}{\frac{d\overline{\Phi}_\textrm{PP,dec}}{dE}}
\newcommand{\sppterm}{d\overline{\Phi}_\textrm{PP}/dE}
\newcommand{\sigmaJ}{\sigma_J}
\newcommand{\Nonij}{{N_{\mathrm{ON},ij}}}
\newcommand{\Noffij}{{N_{\mathrm{OFF},ij}}}
\newcommand{\Nbins}{N_\mathrm{bins}}
\newcommand{\gij}{g_{ij}}
\newcommand{\goffij}{g_{ij}^{OFF}}
\newcommand{\bij}{b_{ij}}
\newcommand{\fij}{f_{ij}}
\newcommand{\tauobsi}{\kappa_{\mathrm{obs},i}}
\newcommand{\sigmataui}{\sigma_{\kappa,i}}
\newcommand{\sigmatausys}{\sigma_{\kappa}^{sys}}
\newcommand{\sigmataustat}{\sigma_{\kappa}^{stat}}
%%% OLD
\newcommand{\Eminj}{{E'_{\mathrm{min},j}}}
\newcommand{\Emaxj}{{E'_{\mathrm{max},j}}}
%%% NEW
\newcommand{\epMinj}{{E'_{\mathrm{min},j}}}
\newcommand{\epMaxj}{{E'_{\mathrm{max},j}}}
%%%
\newcommand{\MNRAS}{Mon. Not. Roy. Astron. Soc. }
%\newcommand{\Comment}[1]{{\color{red}{#1}}}
\newcommand{\atot}{ A_\mathrm{tot}}
\newcommand{\eff}{\epsilon}
\newcommand{\psf}{\mbox{Point Spread Function}}
\newcommand{\bpt}{\bp_\mathrm{tel}}
\newcommand{\bps}{\bp_\mathrm{src}}
\newcommand{\pdfE}{f_E}
\newcommand{\pdfP}{{f_\bp}}
\newcommand{\pdfTheta}{f_\theta}
\newcommand{\fluxunits}{cm$^{-2}$ s$^{-1}$ TeV$^{-1}$}
\newcommand{\difffluxunits}{\fluxunits\, sr$^{-1}$}
\newcommand{\taui}{\tau_i}
\newcommand{\muij}{\mu_{ij}}
\newcommand{\tauij}{\tau_{ij}}
\newcommand{\kij}{\kappa_{ij}}
\newcommand{\RiCR}{R_i^\mathrm{CR}}
\newcommand{\RiX}{R_i^\mathrm{X}}
\newcommand{\RiGDE}{R_i^\mathrm{GDE}}
\newcommand{\Rmin}{R_\mathrm{min}}
\newcommand{\Rmax}{R_\mathrm{max}}
\newcommand{\RminCR}{R_\mathrm{min}^\mathrm{CR}}
\newcommand{\RmaxCR}{R_\mathrm{max}^\mathrm{CR}}
\newcommand{\RminGDE}{R_\mathrm{min}^\mathrm{GDE}}
\newcommand{\RmaxGDE}{R_\mathrm{max}^\mathrm{GDE}}
\newcommand{\dNdE}{\frac{dN}{dE}}
\newcommand{\dJdp}{\frac{dJ}{d\Omega}}
\newcommand{\dJdpp}{\frac{dJ}{d\Omega'}}
\newcommand{\Jann}{J_\mathrm{ann}}
\newcommand{\Jdec}{J_\mathrm{dec}}
\newcommand{\dJdecdpp}{\frac{dJ_\mathrm{dec}}{d\Omega'}}
\newcommand{\Jannsmooth}{\bar{J}_\mathrm{ann}}
\newcommand{\dJdpann}{\frac{d\Jann}{d\Omega}}
\newcommand{\dJdthetaann}{\frac{d\Jann}{d\theta}}
\newcommand{\dJdpdec}{\frac{d\Jdec}{d\Omega}}
\newcommand{\diffJunits}{\Junits\, sr$^{-1}$}
\newcommand{\Dunits}{GeV cm$^{-2}$}
\newcommand{\diffDunits}{\Dunits\, sr$^{-1}$}
\newcommand{\rhounits}{GeV cm$^{-3}$}
\newcommand{\ttbar}{t\bar{t}}
\newcommand{\Nbk}{b}
\newcommand{\Noff}{N_\mathrm{OFF}}
\newcommand{\Non}{N_\mathrm{ON}}
\newcommand{\Rbk}{\frac{d\bar{b}}{dtdE'd\bp'}}
\newcommand{\Roff}{\frac{dN_\mathrm{OFF}}{dtdE'}}
\newcommand{\Tobs}{T_\mathrm{obs}}
\newcommand{\Emin}{E_\mathrm{min}}
\newcommand{\Emax}{E_\mathrm{max}}
\newcommand{\Emini}{{E_{\mathrm{min},i}}}
\newcommand{\Emaxi}{{E_{\mathrm{max},i}}}
%\newcommand{\hatsv}{\widehat{\langle \sigma \mathit{v} \rangle}}
%\newcommand{\hatnu}{\hat{\bm{\nu}}}
%\newcommand{\data}{\bm{\mathcal{D}}}
\newcommand{\NEbins}{N_{E'}}
\newcommand{\NPbins}{N_{\bp'}}
%\newcommand{\gij}{g_{ij}}
%\newcommand{\bij}{b_{ij}}
\newcommand{\bijCR}{b_{ij}^\mathrm{CR}}
\newcommand{\bijGDE}{b_{ij}^\mathrm{GDE}}
\newcommand{\bijX}{b_{ij}^\mathrm{X}}
%\newcommand{\Nonij}{{N_{\mathrm{ON},ij}}}
\newcommand{\Nij}{{N_{ij}}}
%\newcommand{\Noffij}{{N_{\mathrm{OFF},ij}}}
%\newcommand{\Jobs}{J_\mathrm{obs}}
\newcommand{\tauobs}{\tau_\mathrm{obs}}
%\newcommand{\sigmaJ}{\sigma_J}
\newcommand{\sigmatau}{\sigma_\tau}
\newcommand{\sigmak}{\sigma_\kappa}
\newcommand{\tauDM}{\tau_\mathrm{DM}}
\newcommand{\tauDMSen}{\tau_\mathrm{DM|2.71}}
\newcommand{\FoV}{\mbox{FoV}}
\newcommand{\GeV}{\mbox{GeV}}
\newcommand{\TeV}{\mbox{TeV}}
\newcommand{\muG}{\mu\mbox{G}}
\newcommand{\nutau}{$\nu_\tau$~}
\newcommand{\nutaus}{$\nu_\tau$s~}

\usepackage{lineno}
%\linenumbers


\usepackage{fullpage}

\input{add/acro.tex}
\makeglossaries
